Alignment-Enriched Tuning for Patch-Level Pre-trained Document Image Models

Alignment between image and text has shown promising improvements on patch-level pre-trained document image models. However, investigating more effective or finer-grained alignment techniques during pre-training requires a large amount of computation cost and time. Thus, a question naturally arises: Could we fine-tune the pre-trained models adaptive to downstream tasks with alignment objectives and achieve comparable or better performance? In this paper, we propose a new model architecture with alignment-enriched tuning (dubbed AETNet) upon pre-trained document image models, to adapt downstream tasks with the joint task-specific supervised and alignment-aware contrastive objective. Specifically, we introduce an extra visual transformer as the alignment-ware image encoder and an extra text transformer as the alignment-ware text encoder before multimodal fusion. We consider alignment in the following three aspects: 1) document-level alignment by leveraging the cross-modal and intra-modal contrastive loss; 2) global-local alignment for modeling localized and structural information in document images; and 3) local-level alignment for more accurate patch-level information. Experiments on various downstream tasks show that AETNet can achieve state-of-the-art performance on various downstream tasks. Notably, AETNet consistently outperforms state-of-the-art pre-trained models, such as LayoutLMv3 with fine-tuning techniques, on three different downstream tasks.

==> Tables/table_1_3.tex <==
% \begin{table}[t]
%     \centering
%     \small
%     \label{tab:sota}
%     \begin{tabular}{l|c}
%     \toprule
%      \multirow{2}{*}{\bf Model} & \bf RVL-CDIP-1    \\
%      & \bf Accuracy$\uparrow$ \\
%      \midrule
%       $\textrm{BERT} $~\cite{devlin2019bert}   & 89.81  \\
%       $\textrm{RoBERTa} $~\cite{liu2019roberta} &  90.06  \\
%       $\textrm{LayoutLMv2}$~\cite{xu-etal-2021-layoutlmv2}   (G)  &  95.25 \\

%       LayoutLMv3  & 95.44 \\
%      & Ours  & - \\
     
%       $\textrm{BERT} $~\cite{devlin2019bert}   & 89.92  \\
%       $\textrm{RoBERTa} $~\cite{liu2019roberta}  & 90.11  \\
%       $\textrm{LayoutLMv2}$~\cite{xu-etal-2021-layoutlmv2}  (G)  & 95.64 \\

%      LayoutLMv3 & 95.93 \\
%       Ours & -\\
     
%      \bottomrule
    
%     \end{tabular}
%     \caption{
%     \small
%     TBD
%     }
% \end{table}
